Mitigation of Coincident Peak Charges via Approximate Dynamic Programming

A significant portion of a consumer's annual electrical costs can be made up of coincident peak charges: a transmission surcharge for power consumed when the entire system is at peak demand. This charge occurs only a few times annually, but with per-MW prices orders of magnitudes higher than non-peak times. While predicting the moment of peak demand charges over the course of the entire billing period is possible, optimal cost mitigation strategies based on these predictions have not been explored. In this paper we cast coincident peak cost mitigation as an optimization problem and analyze conditions for optimal and near-optimal policies for mitigation. For small consumers we use approximate dynamic programming to first show the existence of a near-optimal policy and second train a neural policy for curtailing coincident peak charges when subject to ramping constraints.

==> background.tex <==
\section{Background}
\label{sec:background}




 % have studied the impact of CP charges and response of businesses to ERCOT CP warning signals. The authors found that businesses likely respond to potential CP's by reducing consumption by 4\% on average but lack temporal flexibility to do so at any given time. Lack of demand flexibility coupled with broad CP warning periods means more temporally precise curtailment efforts are needed if CP costs are to be avoided.

% In this paper we develop a demand curtailment methodology to compare the effectiveness of two CP prediction strategies: one based on historical averages and a feed-forward neural network (NN) based on historical data and weather forecasts. By treating system demand as a random variable, rather than forecasting load directly, we propose curtailing power as a function of a predicted cumulative distribution function (CDF) value. We show for a hypothetical business utility model optimizing power consumption in 2017, using a predicted CDF exceeds 97\% of a perfect CP predictor, with the NN model exceeding the performance of a model based on a historically averaged CDF.
%
%Our primary contributions are 1) the direct utilization of weather forecast data in CP prediction, 2) the formulation of an optimization program which relaxes predicting strictly binary and rare CP events directly and 3) the development of a empirical CDF based CP predictor suited for the optimization program for CP cost arbitrage.

%The rest of our paper is organized as follows: Sec.~\ref{sec:problem} outlines a simple optimization problem for a business subject to CP charges. We state an equivalent formulation utilizing the CDF of system demand values. Sec.~\ref{sec:solution} describes our solution framework utilizing a historical average based and a neural network based CP predictor. Sec.~\ref{sec:results} collates our prediction results, followed by some concluding remarks in Sec.~\ref{sec:conclusion}.

%Coincident peak (CP) charges are a pricing mechanism used by some electrical utilities and system operators to incentivize customers to reduce consumption during system demand peaks~\cite{zarnikau2013response, ercot4cp}. Since a CP charge is on the order of 100 times of regular electricity prices~\cite{puctrates,liu2013data}, it accounts for a significant portion (upwards of 20\%~\cite{liu2013data}) of a business' total annual electrical costs. The Public Utility Commission of Texas (PUCT) for example, levies coincident peak charges annually through a voluntary program during each of the summer months to set transmission fees for participating consumers \cite{puctrates}. In exchange for participation, consumers benefit from discounted electrical rates at all other times. Other CP charging schemes---such as those where utilities announce an upcoming peak ahead of time---are also used, however we are interested in CP charging schemes where the peak is observed \emph{after the fact}.

%For a business to reap such CP charge savings, the challenge lies in predicting when a peak will occur. A business would need to predict the \emph{system-wide demand}, which is not normally done at the customer level. Consequently a system operator typically provides warning signals such as the expected system peak demand or when a peak is expected to occur. Current literature on CP charges focuses on how business can utilize these signals.

%These warning signals sent by system operators, however, are not always reliable. For example,  ERCOT estimates monthly system peak demands via quantile regression \cite{ercotloadforecast} to provide a basis for warning signals. But in 2017, the actual ERCOT peak loads were roughly 4,000 MW less than predicted value, leading to business under-curtailing their load~\cite{ercotloadforecast}. To avoid these type of errors, some other operators provide more conservative signals. For example, Fort Collins PUD typically sends out warning signals for 10 days of the month, usually with only 5 to 10 minutes of lead time. Although these signals are useful to make load curtailment decisions~\cite{liu2013data}, their frequency, high false alarm rates, and short lead time is undesirable and may lead to user fatigue.

  % The authors of \cite{liu2013data} develop a model for data center workload scheduling within the Fort Collins PUD which utilizes the distributor's CP warning signals provided to consumers. Since CP charges are billed based on demand inside a one hour period, Fort Collins PUD warning signals are quite broad and highly variable: upwards of 10 days per month, for 3 consecutive hours on average, and with 5 to 10 minutes of advance notice \cite{liu2013data}, for a single monthly occurrence.%Peak detection or prediction in time series is a difficult task and covers a broad spectrum of problems \cite{gupta2014outlier}. For the purpose of CP charge arbitrage, a consumer is required to predict if a value in the near future will be maximal over a finite time horizon. Variations on peak value prediction over a fixed time horizon are commonplace in finance \cite{mcneil2000estimation}, utilizing an extreme value theory perspective on probability distribution tails. The finite time horizon for a CP however, is not rolling, as is the case in most relevant time series peak detection literature.

%Both works \cite{zarnikau2007industrial} and \cite{zarnikau2013response} showed that businesses likely curtail their demand if enough time is given before the occurs. In this paper we present a framework where a business can use open source data to make curtailment decisions up to 24 hours in advance. Instead of trying to provide a binary forecast of whether the system peak would occur at a given time, we use a ``softer'' decision rule: we estimate the cumulative distribution function~(CDF) of the load. This information provides a likelihood of the peak occurring and a business can adjust its demand according to this likelihood. Specifically, we train a neural network using open source historical load values, timing information~(e.g., day of the week) and weather data. We show that this neural network out performs conventional CP prediction methods based on load forecasting.



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


